Implicit Regularization for Multi-label Feature Selection

In this paper, we address the problem of feature selection in the context of multi-label learning, by using a new estimator based on implicit regularization and label embedding. Unlike the sparse feature selection methods that use a penalized estimator with explicit regularization terms such as $l_{2,1}$-norm, MCP or SCAD, we propose a simple alternative method via Hadamard product parameterization. In order to guide the feature selection process, a latent semantic of multi-label information method is adopted, as a label embedding. Experimental results on some known benchmark datasets suggest that the proposed estimator suffers much less from extra bias, and may lead to benign overfitting.

==> table_comparison.tex <==
\begin{table*}%{p{2.2cm}ccccccc}
	\centering
	\caption{Experimental results of comparing approaches (mean$\pm$std. deviation) on the ten  datasets over three metrics. ( $\downarrow$: the smaller the better; $\uparrow$ : the larger the better). The marker $\bullet$/$\circ$ indicates whether mFSIR is superior/inferior to the other method. win/tie/loss counts of pairwise \textit{t}-test (at 1\% significance level) between mFSIR and each comparing approach. A tie is counted and no marker is given.}
	\scalebox{0.9}{
	\begin{tabular}{p{2.7cm}cccccc}
				\hline
				\hline
	   & \multicolumn{5}{c} {Hamming Loss $\downarrow$}\\
				\cline{2-6}
				\multirow{-2}{*}{Dataset}	&MIFS&MICO&GRRO&LassoNet&mFSIR\\
		\hline
		
        %Birds&.052$\pm$.000$\circ$&.058$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.053$\pm$.001\\
		
		bibtex&.011$\pm$.000$\circ$&.018$\pm$.014$\bullet$&.015$\pm$.000$\circ$& .980$\pm$.001$\bullet$&.017$\pm$.000\\
		
		%Bookmarks&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
        
		%CAL500&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		Corel16k&.023$\pm$.000$\circ$&.052$\pm$.000$\bullet$&.021$\pm$.000$\circ$& .978$\pm$.001$\bullet$&.024$\pm$.000\\
		
		Delicious&.019$\pm$.001$\bullet$&.022$\pm$.000$\bullet$&.020$\pm$.000$\bullet$&.980$\pm$.000$\bullet$&.018$\pm$.000\\
		
	emotions&.341$\pm$.000$\bullet$&.269$\pm$.029$\bullet$&.273$\pm$.000$\bullet$& .729$\pm$.027$\bullet$&.252$\pm$.006\\
		
	Enron&.324$\pm$.000$\bullet$&.360$\pm$.001$\bullet$&.228$\pm$.000$\bullet$& .937$\pm$.002$\bullet$&.056$\pm$.001\\
		
       %Eurlex-sm&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
	   %genbase&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		%Imdb&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		language log&.020$\pm$.000$\circ$&.289$\pm$.001$\bullet$&.291$\pm$.000$\bullet$& .978$\pm$.001$\bullet$&.165$\pm$.002\\
		
		%Mediamill&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		medical&.017$\pm$.000$\circ$&033$\pm$.000$\circ$&.011$\pm$.000$\circ$& .981$\pm$.003$\bullet$&.034$\pm$.000\\
		
        %Nus-Wide BoW&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		%rcv1-s1&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\

		scene&.172$\pm$.000$\bullet$&.161$\pm$.006$\bullet$&.245$\pm$.000$\bullet$& .799$\pm$.009$\bullet$&.117$\pm$.003\\
		
		%slashdot&.177$\pm$.000$\bullet$&.175$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		tmc2007&.137$\pm$.001$\bullet$&.165$\pm$.000$\bullet$&.103$\pm$.000$\bullet$&.920$\pm$.006$\bullet$&.080$\pm$.000\\
        Yeast&.205$\pm$.000$\circ$&.230$\pm$.011$\bullet$&.312$\pm$.000$\bullet$& .744$\pm$.011$\bullet$&.212$\pm$.001\\
        \textbf{win/tie/loss counts for mFSIR} &\textbf{5/0/5}&\textbf{9/0/1}&\textbf{7/0/3}&\textbf{10/0/0}&-\\
	\hline
	   & \multicolumn{5}{c} {Ranking loss $\downarrow$}\\
				\cline{2-6}
				\multirow{-2}{*}{Dataset}	&MIFS&MICO&GRRO&LassoNet&mFSIR\\
		\hline
		
        %Birds&.208$\pm$.000$\circ$&.410$\pm$.007$\circ$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.420$\pm$.020\\
		
		bibtex&.218$\pm$.000$\circ$&.380$\pm$.001$\circ$&.470$\pm$.000$\circ$& .818$\pm$.020$\bullet$&.568$\pm$.003\\
		
		%Bookmarks&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
        
		%CAL500&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		Corel16k&.136$\pm$.000$\circ$&.409$\pm$.001$\circ$&.392$\pm$.016$\circ$& .797$\pm$.008$\bullet$&.756$\pm$.001\\
		
		Delicious&.260$\pm$.000$\circ$&.374$\pm$.001$\circ$&.289$\pm$.003$\circ$& .822$\pm$.012$\bullet$&.721$\pm$.002\\
		
	emotions&.452$\pm$.001$\bullet$&.311$\pm$.062$\bullet$&.281$\pm$.006$\bullet$&.743$\pm$.053$\bullet$&.271$\pm$.006\\
		
		Enron&.357$\pm$.000$\circ$&.368$\pm$.001$\circ$&.264$\pm$.005$\circ$& .877$\pm$.005$\bullet$&.615$\pm$.010\\
		
       %Eurlex-sm&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
	   %genbase&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		%Imdb&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		language log&.170$\pm$.000$\circ$&.314$\pm$.001$\bullet$&.362$\pm$.023$\bullet$& .768$\pm$.029$\bullet$&.312$\pm$.005\\
		
		%Mediamill&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		medical&.098$\pm$.001$\circ$&.111$\pm$.001$\circ$&.081$\pm$.011$\circ$& .958$\pm$.014$\bullet$&.626$\pm$.021\\
		
        %Nus-Wide BoW&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		%rcv1-s1&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\

		scene&.125$\pm$.003$\bullet$&.245$\pm$.015$\bullet$&.220$\pm$.010$\bullet$& .747$\pm$.020$\bullet$&.105$\pm$.004\\
		
		%slashdot&.156$\pm$.010$\bullet$&.406$\pm$.005$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		tmc2007&.222$\pm$.000$\circ$&.268$\pm$.001$\circ$&.149$\pm$.004$\circ$& .900$\pm$.023$\bullet$&.324$\pm$.003\\
		
        Yeast&.182$\pm$.007$\circ$&.316$\pm$.018$\circ$&.297$\pm$.003$\circ$& .740$\pm$.013$\bullet$&.433$\pm$.005\\
        \textbf{win/tie/loss counts for mFSIR} &\textbf{2/0/8}&\textbf{3/0/7}&\textbf{3/0/7}&\textbf{10/0/0}&-\\
%****	   \hline
%****	   & \multicolumn{6}{c} {Average precision $\uparrow$}\\
%****				\cline{2-7}
%****				\multirow{-2}{*}{Dataset}&MIFS&MICO&GRRO&LassoNet&GD&mFSIR\\
%****		\hline
		
        %Birds&.690$\pm$.000$\circ$&.144$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.189$\pm$.010\\
		
		%****bibtex&.510$\pm$.000$\circ$&.123$\pm$.001$\circ$&.058$\pm$.003$\bullet$& .325$\pm$.045$\circ$&.000$\pm$.000$\bullet$&.103$\pm$.002\\
		
		%Bookmarks&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
        
		%CAL500&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		%****Corel16k&.233$\pm$.001$\circ$&.042$\pm$.001$\circ$&.341$\pm$.010$\circ$& .230$\pm$.025$\circ$&.000$\pm$.000$\bullet$&.036$\pm$.000\\
		
		%****Delicious&.544$\pm$.001$\circ$&.097$\pm$.000$\circ$&.599$\pm$.020$\circ$& .208$\pm$.024$\circ$&.000$\pm$.000$\bullet$&.071$\pm$.000\\
		
		%****emotions&.555$\pm$.002$\bullet$&.682$\pm$.050$\circ$&.511$\pm$.003$\bullet$& .720$\pm$.045$\circ$&.000$\pm$.000$\bullet$&.582$\pm$.012\\
		
		%****Enron&.310$\pm$.000$\circ$&.229$\pm$.000$\circ$&.510$\pm$.020$\circ$& .565$\pm$.023$\circ$&.000$\pm$.000$\bullet$&.182$\pm$.005\\
		
       %Eurlex-sm&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
	   %genbase&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		%Imdb&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		%****language log&.305$\pm$.000$\bullet$&.212$\pm$.001$\bullet$&.168$\pm$.018$\bullet$& .267$\pm$.013$\bullet$&.000$\pm$.000$\bullet$&.433$\pm$.004\\
		
		%Mediamill&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		%****medical&.604$\pm$.002$\circ$&.403$\pm$.001$\circ$&.652$\pm$.001$\circ$& .725$\pm$.077$\circ$&.000$\pm$.000$\bullet$&.210$\pm$.012\\
		
        %Nus-Wide BoW&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		%rcv1-s1&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\

		%****scene&.673$\pm$.005$\bullet$&.651$\pm$.018$\bullet$&.700$\pm$.012$\bullet$& .632$\pm$.023$\bullet$&.000$\pm$.000$\bullet$&.748$\pm$.010\\
		
		%slashdot&.554$\pm$.002$\bullet$&.358$\pm$.002$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		%****tmc2007&.440$\pm$.000$\circ$&.199$\pm$.001$\bullet$&.699$\pm$.003$\circ$& .698$\pm$.051$\circ$&.000$\pm$.000$\bullet$&.326$\pm$.002\\
		
        %****Yeast&.745$\pm$.007$\circ$&.665$\pm$.020$\circ$&.314$\pm$.006$\bullet$& .657$\pm$.014$\circ$&.000$\pm$.000$\bullet$&.429$\pm$.003\\
        %****\textbf{win/tie/loss counts for mFSIR} &\textbf{3/0/7}&\textbf{3/0/7}&\textbf{5/0/5}&\textbf{2/0/8}&\textbf{0/0/0}&-\\
	\hline 
	   & \multicolumn{5}{c} {Macro-averaging AUC $\uparrow$}\\
				\cline{2-6}
				\multirow{-2}{*}{Dataset}	&MIFS&MICO&GRRO&LassoNet&mFSIR\\
		\hline
		
        %Birds&.410$\pm$.000$\circ$&.131$\pm$.002$\circ$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.016$\pm$.002\\
		
		bibtex&.518$\pm$.000$\circ$&.036$\pm$.018$\bullet$&.049$\pm$.002$\bullet$& .762$\pm$.034$\circ$&.156$\pm$.004\\
		
		%Bookmarks&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
        
		%CAL500&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		Corel16k&.034$\pm$.000$\bullet$&.011$\pm$.001$\bullet$&.483$\pm$.021$\circ$& .607$\pm$.030$\circ$&.112$\pm$.001\\
		
		Delicious&.602$\pm$.001$\circ$&.063$\pm$.000$\bullet$&.611$\pm$.003$\circ$& .618$\pm$.049$\circ$&.099$\pm$.003\\
		
		emotions&.252$\pm$.016$\bullet$&.536$\pm$.067$\circ$&.563$\pm$.008$\circ$& .771$\pm$.027$\circ$&.510$\pm$.015\\
		
		Enron&.161$\pm$.000$\bullet$&.135$\pm$.001$\bullet$&.638$\pm$.001$\circ$& .663$\pm$.025$\circ$&.383$\pm$.004\\
		
       %Eurlex-sm&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
	   %genbase&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		%Imdb&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		language log&.221$\pm$.000$\bullet$&.115$\pm$.005$\bullet$&.119$\pm$.002$\bullet$& .597$\pm$.021$\circ$&.358$\pm$.012\\
		
		%Mediamill&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		medical&.156$\pm$.002$\bullet$&.313$\pm$.055$\circ$&.351$\pm$.005$\circ$& .896$\pm$.044$\circ$&.292$\pm$.011\\
		
        %Nus-Wide BoW&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		%rcv1-s1&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\

		scene&.673$\pm$.005$\bullet$&.813$\pm$.001$\circ$&.795$\pm$.009$\circ$& .772$\pm$.020$\circ$&.663$\pm$.011\\
		
		%slashdot&.452$\pm$.000$\bullet$&.219$\pm$.002$\bullet$& .000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000$\bullet$&.000$\pm$.000\\
		
		tmc2007&.436$\pm$.000$\bullet$&.149$\pm$.000$\bullet$&.847$\pm$.002$\circ$& .785$\pm$.064$\circ$&.497$\pm$.002\\
		
        Yeast&.596$\pm$.001$\circ$&.319$\pm$.046$\bullet$&.320$\pm$.004$\bullet$& .575$\pm$.024$\circ$&.564$\pm$.004\\
        \textbf{win/tie/loss counts for mFSIR} &\textbf{7/0/3}&\textbf{7/0/3}&\textbf{3/0/7}&\textbf{0/0/10}&-\\
        \hline
	    \hline
		\label{tab:results}
	\end{tabular}
	}
\end{table*}



























